Decentralizing Privacy Enforcement for Internet of Things Smart Objects

Internet of Things (IoT) is now evolving into a loosely coupled, decentralized system of cooperating smart objects, where high- speed data processing, analytics and shorter response times are becoming more necessary than ever. Such decentralization has a great impact on the way personal information generated and consumed by smart objects should be protected, because, without centralized data management, it is more difficult to control how data are combined and used by smart objects. To cope with this issue, in this paper, we propose a framework where users of smart objects can specify their privacy preferences. Compliance check of user individual privacy preferences is performed directly by smart objects. Moreover, acknowledging that embedding the enforcement mechanism into smart objects implies some overhead, we have extensively tested the proposed framework on different scenarios, and the obtained results show the feasibility of our approach.

==> DEPRECATED.tex <==
\iffalse
\begin{algorithm} [h!]
\scriptsize{
%\relsize{5}
Let $Pa$ be the only parameter in $Op.Parameters$\;
Let $att$ be the attribute used in the Aggregation statement $Pa.Att$\;
Let $att_new$ be an attribute, initialized empty\;  
Let $s_{new}$ be a new stream, initialized with an empty schema\;
Let newData be the result of the operation performed by $Op$\;
    
	$att_{new}$.name = $att$.name + $Op.Parameters$.name\;
	$att_{new}$.data = newData\;
	$att_{new}$.category = deriveDC(Op, $refAttSet$)\;
	$att_{new}$.PP = $att$.PP\; 
    $att_{new}$.History =   $att.History \bigcup$ createHistoryEntry($att.Category$, $att_new.Category$)\;  
	$s_{new}$.Attributes =  ${att_new}$\;

{\bf Return} $\langle$$s_{new}$$\rangle$\;
}
\caption{{\em Aggregation}(${Op},{s}$) }

\label{alg:aggr}
\end{algorithm}
\fi


\iffalse
\begin{algorithm} [h!]
\scriptsize{
Let Op.Parameters=\{$a_{1}$, $a_{2}$\} be the two attributes used in the Join statement\;
Let $s_{1}.Attributes$ and $s_{2}.Attributes$ be the set of attributes contained in $s_{1}$ and $s_{2}$ schema, respectively\;
Let $newHE$, $newPP$,  and $newDC$ be an history entry, a privacy preference, and a data category elements, respectively,  initialized as empty\;
Let $s_{new}$ be a new stream, initialized with an empty schema\;

$refAttSet$ $=a_{1}$ $\cup$ $a_{2}$\;
$attributeSet$ = $s_{1}.Attributes$ $\cup$ $s_{2}.Attributes$ $\setminus$ $refAttSet$\;
$newPP$ = derivePP(Op, $refAttSet$)\;
$a_{1}$.PP = $newPP$\;
$a_{2}$.PP = $newPP$\;

$newHE$ = createHistoryEntry($refAttSet$.category, $a_1$.category)\; 
$a_{1}$.History = $a_{1}$.History $\bigcup$ $newHE$\;
$a_{2}$.History = $a_{2}$.History $\bigcup$ $newHE$\;

$s_{new}$.Attributes = $attributeSet$ $\bigcup$ $a_{1}$ $\bigcup$ $a_{2}$\;

{\bf Return} $\langle$$s_{new}$$\rangle$\;
}
\caption{{\em Join}(${Op}, s_{1}, s_{2}$) }

\label{alg:join}
\end{algorithm}
\fi

%For operator $\Pi$, Algorithm \ref{alg:proj} takes as input a tuple $s$ and  parameters modeling $\Pi$, e.g. $Op$. The algorithm returns an updated tuple, containing the new attribute(s) generated by the execution of the $\Pi$ operator given in input and containing the updated $pp$, $history$, and $category$ fields associated  with each attribute involved in $\Pi$. 

%For operator $\Sigma$, Algorithm \ref{alg:aggr} takes as input a tuple $s$ and parameters modeling $\Sigma$, e.g. $Op$. The algorithm returns an updated tuple, containing the new attribute generated by the execution of $\Sigma$  and containing the updated $history$ and $category$ fields associated with each attribute involved in $\Sigma$. We want to underline that, by the nature of $\Sigma$  (such as avg(), sum(), etc.), only one parameter is present in $Op.Parameters$ and that parameter $Pa$ has only one element. Thus, Algorithm \ref{alg:aggr} does not derive new privacy preferences for the new attribute. 

%For operator $\Join$, Algorithm \ref{alg:join} takes as input tuples $s_1$, $s_2$, and parameters modeling $\Join$. The algorithm returns an updated tuple, where attributes of tuples $s_1$, $s_2$ not used by $\Join$  remain unchanged, whereas the used  attributes  have an updated $pp$ and $history$ field. In order to update PEASs for attribute(s) used by  $\Join$ , Algorithm \ref{alg:join} exploits previously discussed functions: \textit{derivePP()} and \textit{createHistoryEntry()}. 









%In order to check privacy preferences compliance, Algorithm \ref{alg:CC}  checks every attribute in the resulting stream. In particular, it checks compliance of the $peopleCount$.$pp$.$consumer$ with the given consumer identity (line 5). Let us assume that the consumer is \textit{smart-home-company}.  In this case, the check  returns true.
%Changed it to above to not to compare it with the centralized version.
%The first is  related to the definition of privacy preferences for newly created data. As introduced in Section \ref{sec:background}, in \cite{ourPaper} we have designed a strategy to deal with this issue, based on privacy preference combination. However, the solution proposed in \cite{ourPaper} targets centralized platforms where data process is performed by registered queries, that can be statically analyzed before the execution. Thus, this  cannot be applied as it is in a decentralized IoT environment, where all operations are  locally and independently performed. Thus,  Another challenge in a decentralized scenario  is assuring the satisfaction of constraints specified by the data owner on data fusion (aka, $jac$ and $cdc$ constraints, see Section \ref{sec:background}). The following example clarifies this point.

\iffalse
%\begin{figure}[!t]
 \removelatexerror
  \begin{algorithm}[h!]
\scriptsize{
%\relsize{5}
Let $s_{new}$ be a new tuple, initialized as empty\;

\For{ each $Pa\in Op.Parameters$}
{
    Let $att_{new}$ be an attribute, initialized empty\;
    Let $refAttSet$ be the set of attributes, specified in $Pa.Attributes$\; 
    Let $newData$ be the result of the operation $Pa$\;
	$att_{new}$.name = $Pa.name$\;
	$att_{new}$.data = newData\;
	$att_{new}$.category = deriveDC(Op, $refAttSet$)\;
	$att_{new}$.PP = derivePP(Op, $refAttSet$)\; 
	$att_{new}$.History =  $\bigcup_{att\in Pa.Attributes} att.History \bigcup$ createHistoryEntry($\bigcup_{a\in Pa.Attributes} a.Category$, $att$.category)\;
    $s_{new}$.Attributes = $s_{new}$.Attributes $\cup$ $att_{new}$\; 
}

{\bf Return} $\langle s_{new}\rangle$\;
}
\caption{{\em Projection}(${Op},{s}$) }

\label{alg:proj}
\end{algorithm}
%\end{figure}
\fi





%review 2, comment 7, deleted and added footnote to the previous scenario, as requrested by the reviewer.
\subsection{Varying the percentage of Sensing SOs with privacy preferences}\label{exp4}
Increasing the percentage of sensing SOs with an associated privacy preference will increase  the number of privacy preferences  to be elaborated.  Thus, we expect that this will impact the execution time. In performing these experiments,  we  executed queries in the set \textit{Complex Queries}, and we associate sensing SOs with privacy preferences taken from {\em  Full PP} set. Results of experiments are illustrated in Figure \ref{fig:percentagePSO} for Processor SO \rom{2}, and in Figure \ref{fig:percentageCSO} for Consumer SO scenarios.

\begin{figure} [H]
	\centering
	\includegraphics[width=85mm]{figure/percentagePSO2.png}
	\caption{Varying the number of sensing SOs with associated a PP in Processor SO \rom{2} scenario  \label{fig:percentagePSO}}
\end{figure}

\begin{figure} [H]
	\centering
	\includegraphics[width=85mm]{figure/percentageCSO2.png}
	\caption{Varying the number of sensing SOs with associated a PP in Consumer SO scenario  \label{fig:percentageCSO}}
\end{figure}

As expected, for both the scenarios, having less nodes with privacy preferences implies less time to process. For Processor SO \rom{2}, even in the worst case, where all nodes have an associated privacy preference, overhead is under 0.7ms, thus performance overhead is less than 9\%. Compliance check performed by Consumer SOs always takes less than 0.7 ms. 

==> DEPRECATEDbackground.tex <==
\vspace{-5pt}
\section{Background}\label{sec:background}

%Reviewer 2 - Comment 1 - Part 2
We assume that data generated by smart objects are modelled as data streams. Moreover, we assume that smart objects are able to perform  a set of   SQL-like operations (i.e., projection ($\Pi$), aggregation ($\Sigma$), join ($\Join$) and selection ($\sigma$)) over data streams, as SQL represents the query model adopted by many data processing systems in the IoT domain \cite{iotSql}. These SQL operators are continuously  evaluated on every incoming  tuple, whereas operations like join and aggregation are processed  on groups of tuples organized as sliding windows. 



\vspace{-10pt}
\subsection{Privacy Preferences}
%Reviewer 2 - Comment 1 - Part 1 
Privacy preferences are specified according to the model proposed in \cite{ourPaper},  which  has been designed to cope with two relevant  challenges that IoT ecosystems pose on the management of individual privacy. As such, using the proposed preference an individual is able to pose new constraints in addition to those  on the  common elements of a privacy policy (e.g., purpose, retention, third party). 
 
The first is that, due to the complexity of the data flows among IoT devices and back-end systems, users easily lose the control on how their data are distributed and processed. This is even  made worse considered that data generated by different IoT devices are fused together to infer new information on individuals. To give individual more control on his data we support privacy preferences that make him able to pose conditions on which portion can be collected, for which  usage purpose, how long it can be stored, and by whom  (i.e., like traditional privacy policies and preferences), but also make him able to pose limitation on how the data can be used to derive new information (e.g., as an example by explicitly stating  what cannot be derived from users data by analytics processes). 
The second challenge the privacy model considers is related to the management of new derived data. Indeed, although the privacy preference helps individual at regulating the derivation of
new data, they fail in controlling how these new data will be managed. At this purpose, the privacy model implements a strategy for an automatic definition of new privacy preferences for newly derived data. This strategy has been defined such that the new preference has to be defined taking into account the privacy preferences associated  to each single piece of data used for computing the new derived data.



%\textbf{The definition and design of privacy preferences regulated by considering key requirements of a decentralized privacy enforcement framework. Requirements behind envisaged privacy preferences are, first making users able to state which pieces of their data, can be jointly accessed, composed or aggregated for given purposes and which parties can access to their data. Second requirement is about managing new derived data, as privacy preferences have to be composed by taking into account the privacy preferences of owners of each single piece of data used for computing the new derived data.}




% presented in Definition \ref{def:ip}. %This second case is used for specifying exceptions when purposes are organized into a tree.
Similar to other privacy preference model, in \cite{ourPaper} data access is regulated based on purposes. It is interesting to note that in \cite{ourPaper} both purpose and categories are hierarchically organized as trees. This simplifies the specification of privacy preferences, in that a preference stated for a node in the tree representing purpose/category  (e.g., physical state as category) implicitly holds also for  all nodes in its subtree (e.g., heart beat, blood pressure, etc.). Moreover, besides making  individual able to specify the purposes for which is allowed the data usage, the model aims at making him also able to pose limitation. As such, the  privacy preference allows the specification of those purposes for which the access is explicitly prohibited.  This is represented via an element, called {\em intended purposes -- ip}, which is modeled as pair (\textit{Aip}, \textit{Exc}), stating that: all requests with a purpose that  descends from  elements in \textit{Aip}  are authorized, except for those that descend from any element in \textit{Exc} in the purpose tree.
 

Besides intended purposes, privacy preferences allow users to explicitly state which portions of their personal data can be  combined/aggregated with other data. Such requirements are expressed in terms of allowed/denied data categories, modelled through the so called {\em joint access constraints -- jac}. More formally, a joint access constraint  for an attribute \textit{a}  is a tuple $\langle$\textit{Adc, Exc, ip}$\rangle$, where \textit{Adc} is the set of  data categories that can be jointly accessed with \textit{a},
 \textit{Exc} is a set of data categories that specialize elements in \textit{Adc} and that cannot be jointly accessed, and \textit{ip} is an intended purpose. This constraint specifies that the categories that descend from those specified in \textit{Adc} can be jointly accessed with attribute \textit{a} for the purposes authorized by \textit{ip}, except for those that descend from any element in \textit{Exc}. 
Finally, a privacy preference allows data owners to specify what  cannot be derived from their data by the analytics processes. This is specified through a \textit{category derivation constraint -- cdc}, that specifies a set of data categories \textit{Cdc} that cannot be derived using the data.\footnote{In what follows, we will use the dot notation to refer to specific components of $jac$ and $ip$ elements.}


%\begin{definition} {\bf (Joint Access Constraint)}\label{def:jac} \cite{ourPaper}
%\textbf{Let $a$ be an attribute of a data stream and let $C$ be the data category associated $a$. A joint access constraint $jac$ for a is a tuple $\langle$Adc, Exc, ip$\rangle$, where $Adc$ (allowed data categories) is a set of data categories belonging to $C$, Exc is a set of data categories that specialize elements in $Adc$, and $ip$ is an intended purpose. $jac$ specifies that the categories that descend from those specified in $Adc$ can be jointly accessed with $c$ for the purposes authorized by $ip$, except for those that descend from any element in $Exc$. Elements of the joint access constraint referred as \textit{jac.Adc}, \textit{jac.Exc} and \textit{jac.Ip}.}
%\end{definition}



%Reviewer 2 - Comment 2

It is relevant to note that  privacy preference model proposed in \cite{ourPaper}  has been designed under the assumption that all data generated by a device would be consumed only by the device vendor (or a target consumer specified by the vendor). This assumption might not hold in decentralized scenarios, characterized by the presence of multiple consumers. Here,  data owners should be able to provide  different preferences for different consumer entities (e.g., based on reputation or other criteria).   To cope with this new requirement,  we extend the privacy preference model in \cite{ourPaper}, so as to allow data owners to specify data consumers to which a preference applies.
%identities of authorized consumers explicitly through $consumer$ field within their privacy preferences.
A privacy preference is therefore formally defined as follows:

\begin{definition} {\bf (Privacy preference)}\label{def:pp} %(Extension of \cite{ourPaper}).
A privacy preference $pp$ is a tuple $\langle${$\alpha$, \textit{consumer}, \textit{ip}, \textit{jac}, \textit{cdc}}$\rangle$, where $\alpha$ is an attribute of a data stream generated by a smart object, \textit{consumer}  specifies the set of data consumers authorized to access $\alpha$,  
\textit{ip} specifies the intended purposes for which $\alpha$ can be collected and used, \textit{jac} specifies a joint access constraint, whereas \textit{cdc} is category derivation constraint specifying a set of data categories  which cannot be derived from $\alpha$.
\end{definition}


\begin{table}[H]
    \centering
    \scriptsize 
    \begin{tabular}{|c|c|}
        \hline
        {\bf  Element} & {\bf Abbreviation} \\
		\hline
        \textit{Consumer ids} & \textit{consumer} \\
        \hline
        \textit{Intended Purpose} & \textit{ip} \\
        \hline
        \textit{Allowed intended purposes of ip} & \textit{ip.Aip} \\
        \hline
        \textit{Prohibited intended purposes of ip} & \textit{ip.Exc} \\
        \hline
        \textit{Joint access constraint} & \textit{jac}  \\
        \hline
        \textit{Allowed data categories for jac} & \textit{jac.Adc} \\
        \hline
        \textit{Prohibited data categories for jac} & \textit{jac.Exc} \\
        \hline
        \textit{Intended purposes for jac} & \textit{jac.ip} \\
        \hline
        \textit{Category derivation constraint} & \textit{cdc} \\
        \hline
    \end{tabular}
\caption{Privacy preference elements' notation} \label{tab:ppElements}
\end{table}
%Therefore, a privacy preference, $pp$ for given attribute $\alpha$, is a tuple $\langle${$\alpha$, ip(\textit{Adc, ip.Exc}), jac(\textit{Adc, jac.Exc}), cdc(\textit{cdc})}$\rangle$.




%ADD updated answer from R3.C1 will be put in the END OF THE SECTION, AFTER CORRECTED IN COVER LETTER
%\textbf{We would like to note that, the privacy preference model proposed in \cite{ourPaper}, has been designed as an extension to common privacy practices like: which portion of data can be collected; how long data can be stored in information system of the consumer; for which usage purposes data can be collected  etc.  Privacy preference model proposed in \cite{ourPaper} has been tailored for centralized IoT systems by extending common privacy practices with \textit{joint access constraints} and \textit{category derivation constraints}.  In this proposal we extend the privacy preference model proposed in \cite{ourPaper} to better fit in decentralized IoT systems. However, we acknowledge that, in heterogeneous IoT ecosystem, smart objects might have different privacy practice specifications.  For instance, device vendors may produce their products with only traditional privacy practices. To cope with the heterogeneity of the privacy settings of smart objects, our privacy enforcement mechanism handles missing privacy specifications (e.g., joint access constraint) as if they were set with the most flexible settings by data owners. }


\begin{example}\label{exp:PPCharlotte}
Throughout the paper, we will use as an example  a smart home system. We assume that the smart home is equipped with a smart  heating and  electricity usage control system. The smart heating system is built on top of a network of smart objects  able to sense temperature values from several rooms, adjust temperature, if needed, and share data with the heating  company. The smart electricity usage system relies on a  network of smart objects  able to sense electricity usage data, locally compute  usage trends, and  send them  to the electricity distribution company. %The smart home company is responsible for smart home applications.

We also suppose that a user, say Charlotte, has installed this smart home system in her apartment and that she wants to specify  a privacy preference \textit{pp} for the  temperature data sensed by the system. In particular, 
Charlotte wants to share her data only with \textit{Smart Home Company} and she wants to release the sensed data only for the administration of the heating system. Moreover, she allows temperature data to be joined with the generic information and health data of her smart watch (e.g.,  body temperature) as this  could  help her properly customize  room temperature. 
%is fine that temperature data  is joined with generic information and health data of her smart watch (e.g.,  body temperature) as this  could  help her to properly customize  room temperature. 
Thus, she agrees that  temperature data is joined with generic information and health data for administration purpose. However,  she prefers that from these data it is not possible to derive sensitive information such as her current location in the apartment or the number of persons in the room. To model these requirements, Charlotte can specify  \textit{pp}  as  \textit{$\langle$\textit{temperature}, \{smart-home-company\}, $\langle$\{admin\}, $\emptyset\rangle$, $\langle$\{generic, health\},$\emptyset$, $\langle$\{admin\},$\emptyset\rangle\rangle$, \{sensitive\}$\rangle$}.
\end{example}

As a final note,  it is interesting to highlight  that the additional elements introduced to cope with the new challenges that IoT scenario poses, (i.e., consumer identities, joint access constraint, category derivation constraint), are not mandatory. This provides flexibility to vendors to decide   whether   adhere only to the common privacy practice  (e.g., supporting privacy preferences with purpose, retention, third party elements) or  to exploit  the extended privacy preference so as to provide users with a more complete control on his/her personal data.


\vspace{-10pt}
\subsection{Privacy Preference Derivation}
An interesting feature of the model in \cite{ourPaper} is its ability to associate privacy preferences with new data generated by smart objects. These new privacy preferences are defined  by combining the privacy preferences specified by each owner of smart objects sensing the data involved in the derivation process.   
Privacy preferences are combined by taking the most conservative approach so that the resulting privacy preference satisfies the constraints specified in all the  privacy preferences associated with smart objects involved in the data fusion process. 
More precisely, the composed privacy preference is defined by taking intersection of the \textit{consumer, jac.Adc} and \textit{ip.Aip}, and by taking union of the \textit{jac.Exc, ip.Exc} and \textit{cdc} fields of privacy preferences involved in data fusion. Due to the lack of space, we present the formal definition of the composed privacy preference in Appendix \ref{app:definitions} as Definition \ref{def:composedpp}.


%More precisely, the new privacy preference is defined as the following:  \textit{consumer} component is created as the intersection of each \textit{consumer} fields; the \textit{ip} component is created as the intersection of \textit{Aip} and the union of \textit{Exc} fields of each \textit{ip};  the \textit{jac} is computed as intersection of \textit{Adc} and the union of \textit{Exc} fields of each \textit{jac};  
%\textit{cdc} is generated  as the  union of each \textit{Cdc} in the privacy preferences of data involved in data fusion.
%Composition is performed by taking union of \textit{consumer}, \textit{Cdc} and \textit{Exc} fields of \textit{ip} and {jac} tuples, and by taking intersection of \textit{Aip} and \textit{Adc} fields of \textit{ip} and {jac} tuples.

 




\begin{example} \label{exp:composedPP}
Let  us consider the privacy preference described in Example \ref{exp:PPCharlotte} and let us further suppose that Charlotte also wants to specify  a privacy preference for the electricity usage data. In particular,   Charlotte wants to share her data with \textit{Electricity Company} and \textit{Smart Home Company}. Moreover, she wishes to release the sensed data only for the administration of the electricity usage system, and that she prefers to join this data with generic information for administration purpose, whereas she does not pose any condition on what cannot be derived from her data. Thus,  she specifies the following privacy preference: \textit{$\langle$\textit{electricityUsage}, \{smart-home-company, electricity-company\}, $\langle$\{admin\},$\emptyset\rangle$, $\langle$\{generic\},$\emptyset$, $\langle$\{admin\}, $\emptyset\rangle\rangle$,  $\emptyset\rangle$}.

Let us also assume that the smart home network executes an equi-join on streams containing  the electricity usage and temperature data generated by  Charlotte's smart home system on $id_{room}$ attributes, which we assume to have in both the two streams. Moreover, we assume that $id_{room}$ attribute has associated the same privacy  preferences of temperature and electricity usage in both streams. When performing the join, there is the need to fuse together these two privacy preferences. 	
According to  model in \cite{ourPaper}, the composed privacy preference for $id_{room}$ in the stream containing  temperature data is: 

\textit{$\langle$\textit{$id_{room}$}, \{smart-home-company\}, $\langle$\{admin\}, $\emptyset\rangle$ ,$\langle$\{generic\}, $\emptyset$, $\langle$\{admin\}, $\emptyset\rangle\rangle$, \{sensitive\} $\rangle$}.

This new  privacy preference states that  information on $id_{room}$ can be released only for administration purpose to the Smart Home Company, can be joined with generic data for administration purpose, and sensitive information cannot be derived from this data.
\end{example}


\vspace{-15pt}
\subsection{Smart object taxonomy}\label{sec:taxonomy}
Since the proposed privacy preserving mechanism aims at working at the smart object level, we have first  to detail which kind of IoT devices we are targeting. 
%In particular, we need to classify smart objects based on their capabilities so as to assign to each of them a possible $role$, and corresponding logic function, that this  smart object  has to  play in  the proposed decentralized privacy preference enforcement mechanism. 
In the IoT domain, device capabilities are extremely heterogeneous. In order to identify some common blocks, we have reviewed several standardization recommendations from different organizations  \cite{Nistir, ituStandard}. In accordance with these documentations, we propose a smart objects taxonomy based on the object \textit{smartness}, aka abilities in sensing and processing individual data, as follows: 
%As such,  we classify smartness of a smart object into three levels, according to their processing capabilities, namely: 


%\begin{itemize}\label{smartnessLevels}
-- {\em First Level of Smartness:}\label{level1} 
at this level, devices have  a very limited capacity, being able only to act as  basic sensors, for sensing  data from the environment.   

-- {\em Second Level of Smartness:}\label{level2}
at the second level, devices have a limited capacity and computing power, making them only able to  perform basic operations by their own, like projection and selection, which do not require window-based processes that are working on tuples organized as sliding windows such as join or aggregation.
These devices might  be virtual or physically manufactured, e.g., a field-programmable gate array (FPGA) or hard-coded  devices.  % If we refer to our smart home scenario, an example of smart objects of  this level  are those   collecting the temperature values sensed from all sensors placed in the room.

 

-- {\em Third Level of Smartness:}\label{level3}
at this level,  we group those devices that have enough capacity and computing power for performing  complex operations by their own, including  window-based operations. % on stream of sensed data. If we refer to our smart home scenario, and example of smart object of third level is a Raspberry Pi\footnote{https://www.raspberrypi.org/documentation/}, powerful enough to communicate with multiple sensors, and perform an average function every half an hour (e.g., average temperature).
   
%\end{itemize}

According to this taxonomy, we argue that a {\em smart object (SO)} might play three different roles in the proposed decentralized privacy enforcement:\footnote{We postpone the reader to Section  \ref{sec:enforcement} for details about processes and algorithms implemented for each role.}

%\begin{itemize} \label{soTypes}
    
-- {\em Sensing Smart Objects:} 
    the main objective of this type of  smart objects is sensing data from the environment. Typically,  a  smart object with a first level of smartness will play this role.
        
-- {\em Processor Smart Objects:}
    this type of  smart objects aim at  creating new information from sensed data by performing operations over them. Complexity of these operations  depends on the smartness level of the object. As such, a  smart object with second or third level of smartness will be able to play this role.
    
-- {\em Consumer Smart Objects:}
    a smart object playing this role is in charge of verifying user privacy preferences before sending data to consumers.  This process is called privacy preference compliance (see Section \ref{complianceAnalysis}). 
Such role can be taken by gateway devices, such as Dell Edge Gateways or HPE Edgeline Gateways. 
%and they offer many benefits such as;
%translating communication protocols of heterogeneous devices, transferring data, running queries etc. 
%They also have high resources and computing power. 
%Considering their operational and communication capabilities, and their widely usage, throughout the paper we assume that gateway devices in IoT systems will take consumer smart object role and will perform privacy compliance check.
  
%\end{itemize}


\begin{example}\label{exp:smartObejcts}
To have a more clear picture about roles of {\em smart objects}, let us consider the smart home scenario given in Example  \ref{exp:PPCharlotte}  (see Figure \ref{fig:smarthome}).  In this  scenario, we can classify sensing smart objects as devices used for measuring electricity usage and sensing room temperature, and as  processor smart objects those used to locally aggregate data sensed by sensing SOs, with the purpose of generating trends of electricity usage as well as average rooms temperature.  Finally, smart objects sending collected information to electricity and heating system companies can be categorized  as consumer smart objects, as their main role is to send data to consumers. 

 \begin{figure} [h] 
	\centering
	\includegraphics[width=0.5\textwidth]{figure/smartHome.png}
	\caption{Smart home scenario} \label{fig:smarthome}
\end{figure}

\end{example}





























%Moved to Appendix
\iffalse
\begin{definition}{\bf (Composed privacy preference)} \label{def:composedpp}  (Extension of \cite{ourPaper}).
Let $\alpha$ be an attribute belonging to the output stream generated by a smart object, and let $At$ be the set of attributes from which $\alpha$ is derived. The privacy preference $pp$ = \langle${$\alpha$, \textit{consumer}, \textit{ip}, \textit{jac}, \textit{cdc}}$\rangle$ for $\alpha$ is derived as follows:
\begin{itemize}
\item \textit{consumer} is defined as the union of the ids in the \textit{consumer} field with all privacy preferences associated to all attributes in $At$, that is:  $consumer=\bigcup_{a\in At}a.pp.consumer$
\item  The intended purpose component $ip$ is defined as:
-- $Aip$ (allowed intended purposes) is the intersection of the purposes implied by the \textit{ip}'s allowed intended purposes of all attributes in \textit{At}, that is: $Aip=\bigcap_{a\in At}$ \footnote{Here, dot notation denotes the element of a tuple} $\bigcup_{p \in a.pp.ip.Aip} p^\downarrow$, where $p^\downarrow$ denotes a set composed of \textit{p} and all purposes descending from \textit{p} in the purpose tree. 
--  $Exc$ (prohibited purposes) is the union of the \textit{ip}'s prohibited purposes of the privacy preferences specified for \textit{At}'s attributes, that is:  $Exc=\bigcup_{a\in At} a.pp.ip.Exc$
\item  The joint access constraint \textit{jac}  is defined as:
--  $Adc$ (allowed data categories) is the intersection of the \textit{jac}'s allowed data categories of all attributes in $At$, that is:  $Adc=\bigcap_{a\in At}\bigcup_{c\in a.pp.jac.Adc} c^\downarrow$, where $c^\downarrow$ denotes the set composed of c and all categories that descend from \textit{c} in the data category tree.
--  $Exc$ (exception) is the union of the \textit{jac}'s exceptions specified for all attributes in $At$, that is: \\ $Exc$=$\bigcup_{a\in At}a.pp.jac.Exc$;
-- $ip$ (\textit{jac} intended purposes) is defined following the same criteria of the preference intended purposes, that is:  $ip.Aip$=$\bigcap_{a\in At}\bigcup_{p \in a.pp.jac.ip.Aip}$ $p^\downarrow$, and  $ip.Exc=\bigcup_{a\in At} a.pp.jac.ip.Exc$.
\item The prohibited data categories \textit{cdc} are defined as the union of prohibited data categories specified in the privacy preferences of all attributes in $At$, that is:  $cdc=\bigcup_{a\in At}a.pp.cdc$
\end{itemize}
\end{definition}
\fi
%\begin{definition} {\bf (Privacy preference)}\label{def:pp} (Extension of \cite{ourPaper}).
%A privacy preference $pp$ is a tuple $\langle${$\alpha$, \textit{ip}, \textit{jac}, \textit{cdc}, \textit{consumer}}$\rangle$, where $\alpha$ is an attribute of a data stream generated by a smart object, \textit{ip} specifies the intended purposes for which $\alpha$ can be collected and used, \textit{jac} specifies a joint access constraint, \textit{cdc} is category derivation constraint,\textbf{whereas \textit{consumer} specifies consumer identities that $pp$ regulates data sharing.} specifying a set of data categories  which cannot be derived from $\alpha$.
%\end{definition}
%. may get involved in data processing and 
%. data can be shared with 
%. various entities may get involved in data sharing.
%. that are able to apply their own queries over the data %ability of so, burda ise yaramaz.
%. and other parties may get involved in data processing , %BU motivasyon data-metadata nin birbirine bagli olmasi.
%. where different smart objects may apply their own queries  over the data and other parties may get involved in data processing.
%. moreover data owners should have 
%. flexibility in specifying their preferences, in that he/she might have different  preferences for different consumer entities (e.g., based on reputation or other other criteria).

%Therefore, a privacy preference $pp$ for given attribute $\alpha$, is a tuple $\langle${$\alpha$, \textit{ip}, \textit{jac}, \textit{cdc}}$\rangle$.

%The pair \textit{Aip} -- allowed intended purposes, and \textit{Exc} -- exceptions, is called {\em intended purposes -- ip}, and authorizes the access for all purposes that descend from the elements in \textit{Aip} in the purpose tree, except for those that descend from any element in \textit{Exc}. \textbf{Throughout the paper, elements of the intended purposes referred as \textit{ip.Aip} and \textit{ip.Exc}.}

%More formally, a joint access constraint  for an attribute \textit{a}  is a tuple $\langle$\textit{Adc, Exc, ip}$\rangle$, where \textit{Adc} is the set of allowed data categories, \textit{Exc} is a set of data categories that specialize elements in \textit{Adc}, and \textit{ip} is an intended purpose. This constraint specifies that the categories that descend from those specified in \textit{Adc} can be jointly accessed with attribute \textit{a} for the purposes authorized by \textit{ip}, except for those that descend from any element in \textit{Exc}. \textbf{Throughout the paper, elements of the joint access constraint referred as \textit{jac.Adc}, \textit{jac.Exc} and \textit{jac.Ip}. } 

==> DEPRECATEDsecurity.tex <==
\vspace{-10pt}
\section{Security Analysis}\label{sec:security}
In this section, we provide a discussion on the security  of the proposed framework. Towards this goal, it is relevant to recall that the main purpose of the framework is to enhance  the  privacy of IoT users making them able to set and enforce their privacy preferences. The privacy enforcement mechanism relies on  meta-data (encoding privacy preferences, data categories, and data history), generated by sensing and processor smart objects.

Based on our literature review on  attacks and security threats in the IoT domain \cite{securityDistributedIoT, secPrivCurrent, farooq2015critical} and on our adversary model , we have classified possible attacks under two main categories, namely \textit{communication attacks} and \textit{node compromise attacks}. In what follows, we first present the adversary model and then we discuss how to cope with these attacks. 





\vspace{-5pt}
\subsection{Adversary Model}\label{sec:adversaryModel} 
We assume that sensing  and processor SOs are susceptible to be compromised by adversaries and thus can act maliciously, whereas consumer SOs are  honest, i.e., they  behave as expected according to the proposed algorithms. This assumption is based on the conjecture that IoT gateway devices, such as Dell Edge Gateways\footnote{$dell.com/us/business/p/edge-gateway$}, or HPE Edgeline Gateways\footnote{$hpe.com/emea_europe/en/servers/edgeline-iot-systems$} hosting consumer SOs are securely produced by their manufacturers and have high resources. 
Indeed, as stated by \cite{securityAnalysisIoT}, a vulnerability in the hardware of such devices will inevitably  threat the whole system. Therefore, we assume that device manufactures will do their best in designing secure gateway devices.
Moreover, we assume that an adversary is capable to block and intercept communication, and is also able to overhear, inject and delete messages exchanged between  smart objects, as well as analyze communication patterns. 





\vspace{-5pt}
\subsection{Communication Attacks}\label{sec:comm}
In performing attacks targeting communication between smart objects, perpetrator positions herself in between two parties to eavesdrop or  alter communication,  while parties believe they are communicating directly to each other. In what follows, we examine the most relevant communication attacks, that is, \textit{Denial of Service (DoS)}, \textit{eavesdropping and tampering}, \textit{false data injection}, \textit{impersonation}, and %\textit{traffic analysis}. 



\textbf{Denial of Service}\label{sec:DoS} 
Denial of Service (DoS)  refers to generate a large amount of network traffic to cause unavailability of the network and its resources.  DoS attacks may cause \textit{unavailability} of a subnet of smart objects, by disrupting their resources and blocking valid requests and communication among devices. Our approach relies on machine to machine communication among smart objects, in which the operations of one smart object, e.g., meta-data generation and update, mostly depend on the data sent by another smart object. Thus, such threat will affect the correct execution of the network. However, this does not impact the security of our approach. Indeed, if there is a subnet working properly, privacy enforcement will be done correctly in that subnet, and for blocked parts of the network no data will be sent among smart objects and processed  and thus no privacy threat will happen.
 Additionally, in order to prevent unavailability of smart object subnets, consumer SOs, which are assumed to be trusted, can be equipped with DoS attack prevention mechanisms. 
 %We recall that we assume consumer SOs have trusted hardware and powerful resources. 
For instance, consumer SOs can be equipped with preventive mechanisms (e.g., \cite{ddosPreventiveIoT}), and network monitoring mechanisms (e.g., \cite{networkBehAnalysisP2P}) to record and keep attack information and check the communication packets.  Additionally, consumer SOs can employ  intrusion-detection techniques (e.g., \cite{intrusionIoT}), and will take some actions as response to DoS attacks, like disconnecting infected devices form the subnet, filtering out packets from attackers,  or using firewall to stop the traffic upon identified attackers.



\textbf{Eavesdropping and tampering }
An adversary might aim to capture the communication traffic between smart objects by performing \textit{eavesdropping} attacks. Therefore, eavesdropping may lead to disclosure of private user data. 
In contrast, \textit{tampering}  threatens meta-data integrity by corrupting or altering data. Alteration of meta-data indeed is a serious threat for our mechanism, since privacy of the users is enforced according to the meta-data associated with the user data. 
In order to prevent data disclosure by eavesdropping attacks and alteration of the privacy meta-data by tampering attacks, our framework can be  complemented with lightweight encryption mechanisms. 
Literature offers plenty of work dealing with such encryption mechanisms, like \cite{lightweightEncryption,cipherSecCertf}. 
%Specifically, smart objects can  be complemented with  encryption mechanisms that make use of lightweight cryptographic primitives (e.g., hash, nonce, etc), and encrypt the data and the meta-data before sending them, by ensuring that data can not be disclosed and privacy meta-data  cannot be compromised during the communication.
 





%ELENA_24_10: at the beginning of the section it is stated that we will consider data injection and deletion but here you consider only data injection, you should add data deletion and how to cope with it
%GOKHAN: Fixed
\textbf{Traffic analysis, impersonation, and false data injection} 
In performing \textit{traffic analysis} attacks, a passive network observer analyzes communication patterns among smart objects to infer sensitive information. Traffic analysis attacks can even be performed on encrypted data, as an attacker ignores the content but cares about the communication patterns. %\cite{smartHomeNoCastle}. 
%ELENA_24_10: which smart objects will be complemented with traffic analysis tools? because sensing and processor so can be untrusted,
%GOKHAN: Added.
Traffic analysis attacks can be performed in various way,s such as rate monitoring attacks, time correlation attacks,  id analysis attacks, etc. 
To cope with traffic analysis attacks, consumer SOs will be complemented with a suite of countermeasures, such as uniform data sending rates, introducing random fake data transfer paths, dummy packet injection mechanisms,and anonymous communication schemes \cite{luo2010location}.
%traffic analysis prevention mechanisms such as \cite{deng2004intrusion, luo2010location}, that make use of different prevention techniques such as: uniform data sending rates, introducing random fake data transfer paths, dummy packet injection mechanisms, anonymous communication schemes to cope with different types of traffic analysis attacks 
%ELENA_24_10:  it is not clear what this long list of tools (e.g,, uniform data sending, etc...) can be used for traffic analysis
%GOKHAN: Corrected.
In performing an  \textit{impersonation} attack, an attacker seizes the identity of a legitimate smart object, such as access credentials of the device, and acts on behalf of the legitimate device. 
%ELENA_24_10: you should also explain what is the fake data injection attack
%GOKHAN: Added.
%To cope with fake data injection and impersonation attacks, smart objects can be complemented with authentication mechanisms, such as \cite{lightweightAuthentication,lightweightAuthSO}. 
%ELENA_24_10: this para is not consistent with the one before, first you state that you would like to complement your system with {lightweightAuthentication,lightweightAuthSO} and then you mention 
%zhu2004interleaved,heer2008alpha}, which is confusing
%GOKHAN: Removed the previous and merged with the one below.
Whereas, in performing \textit{fake data injection} attacks an, adversary injects false data to system in order to affect data fusion and correct execution of the smart object network. 
%Such attacks decrease effectiveness of IoT systems, since further operations going to be performed over data are affected.  
Therefore, we plan to complement smart objects with hop-by-hop authentication protocols, such as \cite{heer2008alpha} to prevent false data injection and impersonation attacks.
%As smart objects are susceptible to be compromised and can perform false data injection attack as an insider,










\vspace{-5pt}
\subsection{Node Compromise Attacks}\label{sec:nodeComp} 
In performing node compromise attacks, perpetrator  gains access to a smart object, and may control it to perform malicious activities, like  injecting malicious data \cite{securityAnalysisIoT, iotpot}.
Node compromise attacks can be mainly done through  \textit{node capture} or \textit{node controlling}.


%ELENA_24_10: it is still not clear why cloning and sybil can effect correct execution of our privacy enforcement setting, whereas the other (e.g., selective fw attacks) do not?
%GOKHAN: Added explanation
Two of the most relevant node compromise attack vectors are  \textit{cloning attacks} and \textit{sybil attacks}. 
Cloning attacks can be used to disable and compromise honest smart objects, whereas by performing sybil attacks the whole system might be dominated by an adversary.
In addition to these, we are aware of other types of node compromise attacks on IoT devices, like selective forwarding attacks, however here we focus on cloning and sybil attacks as they can seriously damage correct privacy enforcement. 




 
 
\textbf{Node capture and node controlling}\label{sec:nodeCapture}
Node capture violates user privacy, since after capturing the node an attacker may acquire and extract information from the captured node.
%Therefore, node capture is a serious threat against our mechanism. 
By \textit{node controlling} an attacker can try to gain control over smart objects, and can use captured smart objects to perform various attacks. As such, node controlling threatens meta-data integrity of our mechanism and may interrupt correct execution of the mechanisms via corrupted devices.
For instance, captured and malicious sensing SOs can associate fake privacy meta-data to sensed data, as such they can generate a meta-data with very loose settings for data sharing. 
Secondly, compromised and malicious processor SOs can alter the derivation of  new privacy meta-data with the result of not correctly enforcing privacy requirements of the data owners. In contrast, we assume consumer SOs are honest, therefore they will not be affected by node capture and  controlling attacks. To cope with node compromise attacks in our setting, we plan to complement consumer SOs with intrusion detection systems  (see e.g.,  \cite{intrusionSvelte})  so as  to make them able to analyze the network and detect compromised nodes acting maliciously or violating policies. 





\textbf{Cloning attacks}\label{sec:cloning}
Today, due to distributed and unattended nature of of IoT networks, most of the smart objects are physically unprotected devices and it is easy for an attacker to gain access to them, thus they are susceptible to be physically captured.  Once, a smart object is compromised, adversary can easily clone the smart object, replicate large number of clones and distribute them to the smart object network, an attack which  is known as cloning  or replication attack. Cloned smart objects may generate fake data and affect the correct execution of the smart object network, as well as they  can be used to disable and compromise honest smart objects and thus damage privacy enforcement.
Different approaches have been proposed to deal with cloning attacks, such as approaches making use of Physical Unclonable Functions (PUF) as device level protection by modifications on device hardware \cite{pufIoT}, centralized clone detection approaches based on trusted authorities \cite{cloneCentralDetect},  or distributed clone detection approaches \cite{cloneAttacksDist}.
%ELENA_24_10: which smart objects? consumer? processor?
%GOKHAN: All smart objects. Added "all"
We plan to complement smart objects with a globally aware distributed clone detection protocol \cite{cloneAttacksDist}, since this mechanism has the advantage of not requiring trusted authorities and hardware modifications.
%In particular, smart objects will sign and exchange their claims and will check whether claims they have received from a particular smart object are coherent, in order to detect cloning attack.  




\textbf{Sybil attacks}\label{sec:sybil}
Sybil attacks refer to maliciously manipulating IoT systems with many sybil smart objects that are generated with stolen and fabricated identities \cite{sybilDefenceEvaluation}. 
Sybil attacks are similar to cloning attacks as both are based on stolen identities, however they differ in that, when performing cloning attacks an attacker uses stolen identity to replicate it in several physical nodes, whereas in performing sybil attacks, an attacker node claims several stolen identities. 
%Sybil attacks can be performed to dominate whole system or disseminate spam and malware to honest smart objects \cite{sybilIoT} and thus can effect correct privacy enforcement.
%social graph-based approaches \cite{socialSybil}
For instance, sybil sensing SOs may release fake data to the smart object network, thus affecting its correct execution. Various approaches have been proposed to deal with sybil attacks, such as cryptography based approaches \cite{sybilCryptography}, intrusion detection approaches \cite{intrusionSvelte}, or network based approaches making use of RSS readings \cite{rssiSybil,sybilDetection}. To cope with sybil attacks in our setting, we plan to complement our approach with an hybrid prevention setting, that makes use of both intrusion detection and RSS readings based approaches. 
In particular, we plan to complement consumer SOs with intrusion detection systems \cite{intrusionSvelte} to detect sybils, as we assume they are honest and have enough resources to host intrusion detection systems. Whereas, all smart objects will be complemented with RSS readings based approach \cite{rssiSybil,sybilDetection}, as they offer efficient solutions for resource constrained devices. Such approaches define a threshold value on RSS readings to distinguish legitimate and sybil nodes based on nodes’ behavior in the network.
%In our framework, smart objects will maintain lists of smart objects and RSS values of smart objects that are in their coverage area, and they will define a threshold value to detect sybil smart objects.













%ELENA_20_10:  I do not think we can use the motivation below, becuase now we are considering not only attacks altering metadata (see for instance eavesdropping), so we should state how we can protect from them
%However, traffic analysis and data injection and deletion attacks do not imply alteration of privacy meta-data, they do not imply damage to proposed privacy enforcement mechanism.
%GOKHAN: Deleted the sentence, added discussion
%ELENA_20_10:  why cloning and sybil attacks ae more relevant for our setting? you should explain
%GOKHAN: Fixed
%ELENA_20_10: you should explain why you select this technique
%GOKHAN: Done.
%ELENA_20_10: Add a brief explanation of RSS readings based approaches. 
%GOKHAN:Done
%Additionally, as stated in Section \ref{sec:adversaryModel}, we believe that IoT devices that have safety-critical roles, such as gateway devices, will have good security mechanisms by  design. As such, gateway devices with consumer SO role will regularly get updated with new firmwares and security features. 
%ELENA_20_10:  you should rewrite the para below, because the techniques you mention are just an example of the many techniques that can be used. So you should state that consumer SO can be equipped with standard mechanism for Dos prevention, such as.....
%GOKHAN: Done
%Moreover, protection against sybil and cloning attacks requires to take additional and different measures, which we examine in detail at Section \ref{sec:cloning} and  \ref{sec:sybil}.
%For instance, an adversary may clone an IoT smart object and can hide herself with authentic device and perform malicious activities in the smart object network. 
%There are different solutions proposed in the literature for WSN and IoT against a major threats of node compromise attacks (see e.g.,  node intrusion detection systems \cite{intrusionSvelte}, \cite{adversaryNodeCapWSN}). We recall that, we assume gateway devices take consumer SO role, therefore consumer SOs are able to analyze communication between routers and smart object subnets. Therefore, to cope with node compromise attacks in our setting, we plan to complement consumer SOs with intrusion detection systems so as  to make them able to analyze the network and detect compromised nodes acting maliciously or violating policies. 
%Sybil smart objects can be used to disseminate malware and to compromise honest smart objects (cfr. to Section \label{sec:nodeComp} for further discussion). Moreover, sybil smart objects may spam honest smart objects to drop them from the smart object network and thus decrease the effectiveness of the IoT systems.
%(cfr. to Section \ref{sec:DoS} for further discussion on that). 
%employed only by consumer smart objects as they require high overhead
%putIoT paper ini bi ac, ne ise yariyormus bu puf clonning te bi anlamaya calis, yani physical attack icin falan kullaniliyosa physical attack ayri bi subsection olarak eklenilebilir, puf la korunmaya calislcak vs. denebilir. Dikkat et ona,,yoksa cozum yonetimi olarak TDSC paperini cloneAttacksDist vermek en garantisi cunku, aradaki fark yontem vs. ne ona bak. Ikisini de option oalrak bu subsection sonunda verebilriz.
%, in order to make cloning attacks impracticable, due to costs of creating exact copy of the PUF.
%Bu alttakiler physical attack parti ile alakali, bi bak bakalim bisey cikar mi burdan....
%Physical attack, may lead to interruption of communication among smart objects and block execution of the IoT application. %Additionally, with use of reverse engineering techniques,  adversary may expose of data collected by smart objects.
%Such exposures of data in smart object, may allow attacker to extract information and cryptographic keys stored in the device and inject malware to the device.
%SVELTE: In a Sybil attack an attacker copies several logical identities on one physical node whereas in a cloned identity (CloneID) attack the attacker copies the same logical identity on several physical nodes 
%\cite{cloneAttacksDist}
%1)A clone is considered totally honest by its neighbors . In fact, without global countermeasures, honest nodes cannot be aware of the fact that they have a clone among their neighbors.
%2)To have a large amount of compromised nodes, the adversary does not need to compromise a high number of nodes. Indeed, once a single node has been captured and compromised, the main cost of the attack has been sustained. Making further clones of the same node can be considered cheap.+
%Additionally, we assume that adversary is also capable to capture and control smart objects, in which she is able to perform malicious activities with captured devices.
%ELENA_17_10: What about sensing and processor SOs?
%GOKHAN: Added. 
%Eavesdropping attack does not imply alteration of privacy meta-data however we still consider it as a threat to our approach since it might harm the user privacy due to data disclosure. 
%(presented in Section \ref{sec:adversaryModel})
%ELENA_17_10: I do not understand the sentence below, physical damaging can be seen as a type of node compromise attack
%GOKHAN: I deprecated this sentence, as agreed.
%In addition to these, we are aware of other types of attacks on IoT devices, like physical damaging, however here we only examine attacks threaten the privacy enforcement.
%Our approach consists of IoT smart objects, where communication of smart objects has vital importance for the privacy enforcement. 
%Therefore, due to false meta-data initialization, privacy preferences of the data owners will not be satisfied, and thus our approach will not be able to enforce privacy of the data owners correctly.
%DoS Node Compromise: Secondly threat caused by DoS attack is \textit{node compromise}, where attacker aims to capture and control smart objects. We extensively discuss the node compromise threat in Section \ref{sec:nodeComp}, by analyzing its effects and prevention mechanisms.
%ELENA_10_10: Sybils should be discussed here, rather than in a separate section
%GOKHAN: Added.
%devices can be complemented cryptographic methods, however sensing SOs and processor SOs I, will not be able to perform strong cryptographic operations to secure data. Therefore,
%Distributed Denial of Service (DDoS) refers is a special type of DoS attack where perpetrator uses geographically distributed more than one computers or devices, which s.
%Dolev-Yao: The adversary in this model can overhear, intercept, and synthesize any message and is only limited by the constraints of the cryptographic methods used. In other words: "the attacker carries the message." 
\iffalse
\begin{table*}
    \centering
    \scriptsize 
    \begin{tabular}{|c|c|c|c|}
        \hline
        {\bf Attacks}  & {\bf DDoS} & {\bf MITM} & {\bf Node Compromise}   \\
       % {\bf analysis}  & {} & {\bf Damage} & { \bf dropping } & {\bf Capture}  & { \bf ling} \\
        \hline
     	 & \textit{Unavailability} & \textit{Sniffing}  & \textit{Node Capture}\\
         \textbf{Threats} & \textit{Node Compromise} & \textit{Spoofing}  & \textit{Node Controlling} \\
         &  & \textit{Tampering} & \\
		% & & & \\
        % & & & \\
        \hline

    \end{tabular}
\caption{ Threat Analysis for Proposed Framework: Threat:$\checkmark$, Not Threat:\textit{X}  } \label{tab:sec}
\end{table*}  
\fi
%Presented in Figure \ref{fig:attackDefense}
%\begin{figure*} [h]
%	\centering
%	\includegraphics[width=185mm]{figure/Attack_Privacy_Framework_.png}
%	\caption{Attack defense tree for the privacy enforcement framework \label{fig:attackDefense}}
%\end{figure*}
% To see how to cope with this threats we have first to point out who are the possible attackers, that is,  who can perform these actions. 
%Attacks and threat groups has been in this section, where Table \ref{tab:sec} presents threats. Then, we have to provide discussion on threats by examining their effects on the proposed framework, and how such threats can be handled.  
%our privacy enforcement mechanism will not be altered
%Which implies that congested network and cracked smart objects may harm a subset of the smart objects in the network, which indeed is a threat for our approach. 
%\cite{secDataTransferNodeCapWSN}
%In Wireless Sensor Network (WSN) domain, node compromise attacks has gained much interest, and literature offers interesting works about this attack \cite{nodeCompromiseWSN,secDataTransferNodeCapWSN,adversaryNodeCapWSN}. Similarly, smart objects in IoT domain may also be target of such attacks and susceptible to be compromised \cite{iotpot,securityAnalysisIoT}. Therefore, node compromise attacks  
%literature offers interesting work highlighting that IoT devices may be target of various attacks and susceptible to be compromised \cite{iotpot,securityAnalysisIoT}.
%\cite{compromisedNodeWSN} : Wireless sensor networks are often deployed in unattended environments. Node compromise is the central problem that uniquely characterizes the sensor network’s threat model. So, in this paper a straightforward but effective scheme, SSACH, is presented. SSACH focuses on secure information aggregation in sensor networks that can handle a malicious CH and malevolent sensor nodes. SSACH has been demonstrated to exhibit excellent performance. 
%Node compromise occurs when an attacker, though some subvert means, gains control of a node in the network after deployment. Once in control of that node, the attacker can alter the node to listen to information in the network, input malicious data, cause DOS, black hole, or any one of a myriad of attacks on the network. The attacker may also simply extract information vital to the network’s security such as routing protocols, data, and security keys. Generally compromise occurs once an attacker has found a node, and then directly connects the node to their computer via a wired connection of some sort. Once connected the attacker controls the node by extracting the data and/or putting new data or controls on that node. 
%Sniffing:
%Sniffing refer to listening to a conversation. For example, if you login to a website that uses no encryption, your username and password can be sniffed off the network by someone who can capture the network traffic between you and the web site.
%Any eavesdropping on existing traffic can be called sniffing, for example you can sniff your own traffic using a network sniffer, I think the WireShark is a good tool for this purpose. WireShark does not change the packets and only capure them and display them, this is the meaning of sniffing.
%Spoofing:
%Spoofing refers to actively introducing network traffic pretending to be someone else. For example, spoofing is sending a command to computer A pretending to be computer B. It is typically used in a scenario where you generate network packets that say they originated by computer B while they really originated by computer C. Spoofing in an email context means sending an email pretending to be someone else.
%When someone(or something) try to introduce himself as another person (or another object), this called spoofing, for example there is IP Spoofing, DNS Spoofing etc in IP Spoofing suppose person A send a packet with source address B not A (not himself IP address) to another host. this is a simple IP Spoofing. And inDNS Spoofing A person tries to put his own IP address as the name of a victim host in the DNS server, this is also a simple DNS Spoofing
%-Replay Attacks.. is it related? yeah somehow, but it is not a thread for the system:
%\textit{Eavesdropping}: we also consider traffic analysis: no prob for us
%In \cite{cipherSecCertf}, a lightweight encryption decryption method for ID authentication among nodes in sensor layer.
%\cite{} auth
%\textit{Tampering Attack}
%\textit{Packet Deleting and Injection Attacks:}
%To cope with this issue, we can complement our system with security mechanisms defined so far for wireless sensor networks, RFID,etc.  to secure data exchange among nodes \cite{lightweightAuthentication, iotSecurityHash,lightweightCryptography}.
%it can capture the information, it can corrupt it, and then it can reinject it back into the flow. In other words, it can break down your trust identity to modify traffic in a malicious way. It can also introduce new information into network sessions.
%is very important privacy protection while query execution, mostly depends on data sent by another smart object. Indeed, such threat effects correct execution of the network,
%For correct execution of our privacy enforcement mechanism, communication between smart objects have to be performed securely
%Assuming that smart objects behave honestly, metadata integrity can be compromised only by external attackers during data exchange among SOs.
%We refer the interested reader to  \cite{securityDistributedIoT, securityDistributedIoT,infoSecm2mIoT, systemicApproachIoTSec} for a broader discussion and analysis on possible attacks targeting IoT device communication. 
%In this discussion we assume that sensing, processor and consumer SOs are honest, i.e., they will behave as expected according to the proposed algorithms, and would not intentionally alter metadata. 
%Proposed model does not have node compromise tolerance, since compromised nodes may modify privacy meta-data and let the system lose control over user privacy. Therefore we have to assume nodes are acting honestly, and willing to cooperate privacy enforcement. 
%However, as stated by \cite{securityAnalysisIoT} a vulnerability in the hardware of the IoT device, will inevitably lead to have compromised devices and such situation may threat the whole system. This brings us to think that IoT device manufactures will do their best in designing secure devices \footnote{As an example, Samsung Knox: https://www.samsungknox.com/en}.
%\subsection{Check}
%\textbf{Change: In hardware implementations, chip size and/or energy consumption are the important measures to evaluate the lightweight properties. In software implementations, the smaller code and/or RAM size are preferable for the lightweight applications. From the view of the implementation properties, the lightweight primitives are superior to conventional cryptographic ones, which are currently used in the Internet security protocols, e.g. IPsec, TLS.  }
%\textit{honest but curious}: follows protocol correctly, but possibly tries to infer user information from the managed resources. "For this reason, our model requires that all the resources are being uploaded encrypted and that the metadata uploaded along with each resource do not reveal any information regarding the identity of co-owners."
%\cite{infoSecm2mIoT} Three ways to analyze the existing information security of Internet of Things:
%1) Front-end Sensors and Equipment: 
%- IoT Machine/Perception Nodes in the local security threat and Analysis:  machine/perception nodes are most deployed in the absence of monitoring scenarios, then the attacker can easily access to these devices causing damage %or illegal action by local operators 
%\begin{itemize}
%\item Unauthorized access to data: Stubborn(**dirayetli etc.**) equipments should be used, and two-way authentication mechanism of network and the corresponding encryption algorithm should be designed to prevent from eavesdropping or unauthorized access the data on wireless links.
%\item Threat and Analysis to the Internet: attacker can cause damage of the  transaction information on the m2m user by modifying, inserting, replaying, or deleting the legitimate m2m user data
%\end{itemize}
%\textbf{Attacks targeting Sensing SOs:}
%A sensing SO much likely to be selected as a target by an attacker by considering their limited capabilities (discussed in Section \ref{sec:taxonomy}) and likely sensitive and private data they sense. In proposed privacy preserving mechanism, sensing SOs are entitled to associate the  data category and privacy preferences specified by user as metadata to the data it sense. In such scenario, data and metadata have to be kept confidential securely inside of the sensing SO before sending them as encapsulated within a transaction to processor SOs. Given all, some possible threats over sensing SO are: 
%\textbf{Attacks targeting Processor SOs:}
%As a typical processor SO aggregates and processes data sent from variety of sensing SOs and performs derivation of new privacy
%: unauthorized access 
%\textbf{Attacks targeting Consumer SOs:}
%As discussed previously, main objective of a consumer SO is to decide whether share or not share data by considering compliance of its associated metadata (privacy preferences) and privacy *practice* of to consumer. Injection, compromised device, .......reasons......., in such cases consumer SO will not be able to correctly enforce users privacy preferences.
%Finally, attackers may even use those compromised devices to create a botnet for further DDoS attacks targeting all websites, systems and servers over the Internet, as its already happened recently
%\textbf{ Such smart objects can be target of attacks that may be threat for correctness and integrity of the proposed system. Specifically, dysfunctionality of a Consumer SO may effect privacy preference compliance check (will be discussed in Section \ref{complianceAnalysis}), may led proposed mechanism to lose control of users' privacy.  Additionally, attacks targeting Sensing SOs and Processor SOs may manipulate derivation of privacy metadata (will be discussed in Section \ref{def:sec:peas}) of users' data.  }
%attacker may inference users data with its metadata, signaling data in transmission of wireless link through the physical layer or protocol layer, to achieve denial of service attacks of wireless attacks \cite{infoSecm2mIoT}.
% Other threat of DDoS attack is node capture, and in general \textit{node compromise}. As stated in \cite{iotBotnets}, infected IoT devices are used in DDoS attacks widely by generating a network of bots, aka botnets. Such situation implies that, node capture and controlling may cause generating a new attacker, a zombie device from captured node, and make it part of the botnet to use in new attacks\footnote{http://www.thesecurityblogger.com/largest-ddos-attack-ever-delivered-by-botnet-of-hijacked-iot-devices/}. This threat and its effects is discussed in following Section \ref{sec:nodeComp} in detail.
%To prevent DoS attacks, consumer SOs will be responsible of execution of techniques to monitor and measure DoS attacks (e.g., consumer SOs will record and keep attack information, check and filter out packets, monitor network and device behaviors and use firewalls \cite{ddosPreventiveIoT, preventiveAdapDDoS}). 
%As stated in \cite{iotBotnets}, many IoT devices may not have enough processing power and sufficient memory, aka smartness, therefore the intrusion detection may likely to occur at a gateway device. %As such, consumer SOs may also be used as a gateway device to employ intrusion detection mechanisms, since we assume consumer SOs are trusted and have high capabilities.
%Considering Consumer SOs higher level capabilities comparing low level IoT devices, as discussed in Section \ref{sec:taxonomy}, additional high resource demanding security mechanisms may be employed by Consumer SOs like firewalls. 
%intrusionIoT,decentralizedIntrusion
%As such, we consider only  attacks that compromise metadata integrity, whereas attacks on data confidentiality is out of the scope of this first proposal.
%and table \ref{tab:sec} illustrates attacks and their threats that we examine.
%we propose to use consumer SOs as gateway devices between routers and subnets of the smart object network, consisting of sensing and processor SOs (e.g. the smart home network). We recall that, we assume consumer SOs have trusted hardwares and powerful resources. 
%In order to simplify our adversary model, we ignore the resources an adversary needs to expend in order to attack a system.
 %Please refer to example works from literature \cite{ddosPreventiveIoT, preventiveAdapDDoS} for further discussion and example defense strategies for DoS attacks.
%consumer SOs will be responsible for applying prevention, monitoring and response mechanisms to secure the IoT network.
%Specifically, 
% As stated in \cite{iotBotnets}, if IoT devices are missing from such properties, than consumer SOs will employ \textit{intrusion-detection} techniques .
%\subsubsection{Traffic analysis}
%Traffic analysis attack performed by examining communication patterns of smart objects. Traffic analysis attack can even be performed on encrypted data, as attacker ignores the content but cares about the communication patterns \cite{smartHomeNoCastle}, which threatens privacy of the smart object owners. 
%\subsection{Physical and Cloning attacks}
%\textbf{Today, due to distributed and unattended nature of of IoT, most of the smart objects physically unprotected devices and it's easy for an attacker to gain access to them. Physical attack, may lead to interruption of communication among smart objects and block execution of the IoT application. Moreover, with use of reverse engineering techniques, adversary may expose of data collected by smart objects.
%Lightweight encryption mechanisms, like \cite{lightweightEncryption,cipherSecCertf}. 
%Such exposures of data in smart object, may allow attacker to extract information and cryptographic keys stored in the device and inject malware to the device. Adversary may clone an IoT device and can hide herself with authentic device and perform malicious activities in the smart object network.  In order to protect smart objects against device cloning, we can complement smart objects in our framework with Physical Unclonable Functions (PUF), like as in \cite{pufIoT}, in order to make cloning attacks impracticable, due to costs of creating exact copy of the PUF \cite{pufIoT}}
%Literature offers some interesting work in the field of Wireless Sensor Networks (WSN) and IoT domains highlighting that sensor nodes and IoT smart objects may be target of such attacks and susceptible to be compromised . Node compromise attacks may harm meta-data integrity, may cause incorrect system execution and may allow malicious activities performed in the network. 
%Complexity of the encryption mechanisms  data protection is required for a shorter time span, as discussed previously.
%Therefore, lightweight encryption mechanisms, such as with smaller key sizes, will be enough to protect integrity of the privacy meta-data.
% Eavesdropping attack does not imply alteration of privacy meta-data but since it might harm the user privacy complementing our approach with lightweight encryption mechanisms \cite{lightweightEncryption,cipherSecCertf}, will provide protection against against eavesdropping attacks. 
%We note that, DoS attacks can be performed to compromise smart objects, which is referred as \textit{node compromise} attacks. We examine the node compromise attacks and its threats to our approach in the Section \ref{sec:nodeComp}. 
%ELENA_10_10: the following subsections are not homogeneous. For instance, you have a section on communication attacks, but Dos can be a seen as type of communication attack (that is, they are both node compromise and communication attacks). The same comment applies to sybil attacks, they fall under node compromise attacks.
%you should restructure the section by re-organizing the material as follows:
%\section{Communication attacks}
%put here all the possible attacks on communication (structured into subsections)
%\section{Node compromise attacks}
%put here all the possible attacks on communication (structured into subsections)
%GOKHAN: Corrected.
%\footnote{As an example, Microsoft is developing the project Sopris for secure Internet connected devices: microsoft.com/en-us/research/project/sopris/}
%As such, we focus on attacks  compromising  meta-data integrity (e.g., modification, deletion, etc.), which could invalidate  privacy preferences enforcement. 
%Therefore, in the following we analyze possible attacks that might compromise meta-data integrity.

==> DEPRECATEDtaxonomy.tex <==
\vspace{-10pt}
\section{Smart object taxonomy and roles}\label{sec:taxonomy}


Since the proposed privacy preserving mechanism aims at working at smart object level, we have to first   detail which kind of IoT devices we are targeting. In particular, we need to classify smart objects based on their capabilities so as to assign to each of them a possible $role$, and corresponding logic function, that this  smart object  has to  play in  the proposed decentralized privacy preference enforcement mechanism.
In the IoT domain, capabilities of devices are extremely heterogeneous. In order to identify some common blocks, we have reviewed several standardization recommendations from different organizations  \cite{Nistir, iot-a, ituStandard}. In accordance with these documentations, we propose a smart objects taxonomy based on the object \textit{smartness}, aka abilities in sensing and processing individual data, as follows: 
%As such,  we classify smartness of a smart object into three levels, according to their processing capabilities, namely: 


%\begin{itemize}\label{smartnessLevels}
-- {\em First Level of Smartness:}\label{level1} 
at this level, devices have  a very limited capacity, being able only to act as  basic sensors, for sensing  data from the environment.   

-- {\em Second Level of Smartness:}\label{level2}
at the second level, devices have a limited capacity and computing power, making them able only to  perform basic operations by their own, like projection and selection, which do not require window-based processes. These devices might  be virtual or physically manufactured, e.g., a field-programmable gate array (FPGA) or hard-coded  devices.  % If we refer to our smart home scenario, an example of smart objects of  this level  are those   collecting the temperature values sensed from all sensors placed in the room.

 

-- {\em Third Level of Smartness:}\label{level3}
at this level,  we group those devices that have enough capacity and computing power for performing  complex operations by their own, including  window-based operations. % on stream of sensed data. If we refer to our smart home scenario, and example of smart object of third level is a Raspberry Pi\footnote{https://www.raspberrypi.org/documentation/}, powerful enough to communicate with multiple sensors, and perform an average function every half an hour (e.g., average temperature).
   
%\end{itemize}



A {\em smart object (SO)} might play three different roles in the proposed decentralized privacy enforcement:\footnote{We postpone the reader to Section  \ref{sec:enforcement} for details about processes and algorithms implemented for each role.}


%\begin{itemize} \label{soTypes}
    
-- {\em Sensing Smart Objects:} 
    the main objective of this type of  smart objects is sensing data from environment. Typically,  a  smart object with a first level of smartness will play this role.
        
-- {\em Processor Smart Objects:}
    this type of  smart objects aim at  creating new information from sensed data by performing operations over them. Complexity of these operations  depends on the smartness level of the object. As such, a  smart object with second or third level of smartness will be able to play this role.
    
-- {\em Consumer Smart Objects:}
    a smart object playing this role is in charge of verifying user privacy preferences before sending data to consumers.  This process is called privacy preference compliance and, as it will be discussed in Section \ref{complianceAnalysis},   it  requires to implement a set of algorithms. As such, a smart object with third level of smartness  may play this role.
     
%\end{itemize}


\begin{example}\label{exp:smartObejcts}
To have a more clear picture about roles of {\em smart objects}, let us consider the smart home scenario given in Example     \ref{exp:PPCharlotte}  (see Figure \ref{fig:smarthome}).  In this  scenario, we can classify sensing smart objects as devices used for measuring electricity usage and sensing room temperature, and as  processor smart objects those used to locally aggregate data sensed by sensing SOs, with the purpose of generating trends of electricity usage as well as average rooms temperature.  Finally, smart objects sending collected information to electricity and heating system companies can be categorized  as consumer smart objects, as their main role is to send data to consumers. 

 \begin{figure} [h] 
	\centering
	\includegraphics[width=0.5\textwidth]{figure/smartHome.png}
	\caption{Smart home scenario} \label{fig:smarthome}
\end{figure}

\end{example}



%Table \ref{tab:SmartnessLevels} summarizes, for each smartness level, the operations that objects of that level can perform, the possible roles that can play.


%\begin{table}[h]
 %   \centering
  %  \scriptsize
   % \begin{tabular}{|c|c|c|c|c|c|c|c|}
     %   \hline
    %    {\bf Smart } &  & &  & &  & \textbf{Privacy} & \\
      %  {\bf object} & \textbf{Sense}  & {\bf $\sigma$} & {\bf $\pi$} & {\bf $\Join$ } & {\bf $\Sigma$} & {\bf Preference} & {\bf Role }\\
       % {\bf types} &   &  &  &   &  & {\bf  Compliance } & {}\\
        %\hline
        %\textit{First } &  & &  & &  &  & \\
        % \textit{Smartness } & \textit{ $\checkmark$ } & &  & &  & &Sensing  \\
         % \textit{ Level}&  & &  & &  &  & \\
        % \hline
    %    \textit{Second } &  & &  & &  &  & \\
     %   \textit{Smartness } &  &\textit{ $\checkmark$ } & \textit{ $\checkmark$ } & &  & &Processor SO   \\
       % \textit{Level}&  & &  & &  &  & \\
    %   \hline
     %   \textit{Third }&  & &  & &  & &Processor   \\
      %  \textit{Smartness }&  &\textit{ $\checkmark$ } & \textit{ $\checkmark$ } & \textit{ $\checkmark$ }& \textit{ $\checkmark$ } &\textit{ $\checkmark$ } &Consumer   \\
       % \textit{Level} &  & &  & &  &  & \\
        % \hline
    %\end{tabular}
%\caption{ Summary of Operations and Roles Performed by Smart Object based on its Smartness Level} \label{tab:SmartnessLevels}
%\end{table}   




















